Deep-QPP: A Pairwise Interaction-based Deep Learning Model for Supervised Query Performance Prediction

Motivated by the recent success of end-to-end deep neural models for ranking tasks, we present here a supervised end-to-end neural approach for query performance prediction (QPP). In contrast to unsupervised approaches that rely on various statistics of document score distributions, our approach is entirely data-driven. Further, in contrast to weakly supervised approaches, our method also does not rely on the outputs from different QPP estimators. In particular, our model leverages information from the semantic interactions between the terms of a query and those in the top-documents retrieved with it. The architecture of the model comprises multiple layers of 2D convolution filters followed by a feed-forward layer of parameters. Experiments on standard test collections demonstrate that our proposed supervised approach outperforms other state-of-the-art supervised and unsupervised approaches.

==> figdefs/architecture_detailed.tex <==
\begin{figure*}[t]
\centering
    \subfloat[single channel.]
    {\label{fig:single_channel}
    \includegraphics[width=.4\textwidth,]{figs/single_channel.pdf}}
    \quad
    \subfloat[multi channel (row vector)]
    {\label{fig:multi_row}
    \includegraphics[width=.4\textwidth]{figs/multi_channel_row.pdf}}
    \quad
    \subfloat[multi channel (col vector)]
    {\label{fig:multi_col}
    \includegraphics[width=.4\textwidth]{figs/multi_channel_column.pdf}}
    \quad
    \subfloat[each qterm-doc]
    {\label{fig:each_qterm_doc}
    \includegraphics[width=.4\textwidth]{figs/each_qterm_doc.pdf}}
    \caption{Model variants.}
    \label{fig:model}
\end{figure*}

==> plotdefs/bin_sensitivity.tex <==
\begin{figure}[t]
\centering
\resizebox{0.9\columnwidth}{!}{
   \begin{tikzpicture}
       \begin{axis}[
           title={\textbf{(a) TREC-Robust}},
           xlabel={$p$ (\textbf{Bin-size}}),
           ylabel={\textbf{Metric (Accuracy/$\rho$/$\tau$)}},
           xmin=10, xmax=50,
           ymin=0.45, ymax=1,
           xtick={10,20,30,40,50},
           ytick={0.5,0.6,0.7,0.8,0.9,1},
           legend pos=north east,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=red,
           mark=x,
           ]
           coordinates {(10,0.7949)(20,0.8271)(30,0.8420)(40,0.8063)(50,0.804)};
       %
       \addplot[
           line width=0.5mm,
           color=olive,
           mark=square,
           ]
           coordinates {(10,0.6683)(20,0.7034)(30,0.7404)(40,0.7346)(50,0.7038)};
       %
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=o,
           ]
           coordinates {(10,0.4927)(20,0.5311)(30,0.5434)(40,0.512)(50,0.4731)};
    %   
       \legend{\textbf{Accuracy},\textbf{\pr},\textbf{Kendall's-$\tau$}}
       \end{axis}
   \end{tikzpicture}
% 
   \begin{tikzpicture}
       % \centering
       \begin{axis}[
           title={\textbf{(b) ClueWeb09}},
           xlabel={$p$ (\textbf{Bin-size}}),
           ylabel={\textbf{Metric (Accuracy/$\rho$/$\tau$)}},
           xmin=10, xmax=50,
           ymin=0.15, ymax=1.2,
           xtick={10,20,30,40,50},
           ytick={0,0.2,0.4,0.6,0.8,1},
           legend pos=north east,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=red,
           mark=x,
           ]
           coordinates {(10,0.7635)(20,0.7972)(30,0.8045)(40,0.7907)(50,0.7729)};
       %   
       \addplot[
           line width=0.5mm,
           color=olive,
           mark=square,
           ]
           coordinates {(10,0.4963)(20,0.5442)(30,0.5532)(40,0.5127)(50,0.4836)};
       %
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=o,
           ]
           coordinates {(10,0.2753)(20,0.2984)(30,0.3130)(40,0.3065)(50,0.3004)};
       %
       \legend{\textbf{Accuracy},\textbf{\pr},\textbf{Kendall's-$\tau$}}
       \end{axis}
   \end{tikzpicture}
}
\caption{
\small
Sensitivity of \ours~w.r.t. the bin-size, $p$.
}
\label{fig:bin_compare}
\end{figure}


==> plotdefs/epoch_vs_time.tex <==
\begin{figure}[t]
\centering
\resizebox{1\columnwidth}{!}{
   \begin{tikzpicture}
       \begin{axis}[
           title={\textbf{(a) TREC-Robust}},
           xlabel={\textbf{Epochs}},
           ylabel={\textbf{Cumulative training time (mins.)}},
           xmin=1, xmax=10,
           ymin=1, ymax=70,
           xtick={1,2,3,4,5,6,7,8,9,10},
           ytick={0,10,20,30,40,50,60,70},
           legend pos=north west,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=o,
           ]
           coordinates {(1,1.48)(2,3.00)(3,4.50)(4,5.99)(5,7.51)(6,9.01)(7,10.62)(8,12.26)(9,13.94)(10,15.56)};
       %
       \addplot[
           line width=0.5mm,
           color=orange,
           mark=x,
           ]
           coordinates {(1,5.34)(2,10.68)(3,16.18)(4,21.86)(5,27.86)(6,33.70)(7,39.37)(8,45.21)(9,51.55)(10,57.72)};
       \legend{\textbf{\ours~(SDMQ)},\textbf{\wsup}}
       \end{axis}
   \end{tikzpicture}
%   
    \begin{tikzpicture}
       \begin{axis}[
           title={\textbf{(b) ClueWeb09}},
           xlabel={\textbf{Epochs}},
           ylabel={\textbf{Cumulative training time (mins.)}},
           xmin=1, xmax=10,
           ymin=1, ymax=70,
           xtick={1,2,3,4,5,6,7,8,9,10},
           ytick={0,10,20,30,40,50,60,70},
           legend pos=north west,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=o,
           ]
           coordinates {(1,1.79)(2,3.20)(3,4.89)(4,6.99)(5,8.41)(6,10.20)(7,12.46)(8,13.26)(9,14.94)(10,16.56)};
       %
       \addplot[
           line width=0.5mm,
           color=orange,
           mark=x,
           ]
           coordinates {(1,6.34)(2,11.68)(3,17.18)(4,22.86)(5,28.86)(6,35.70)(7,40.37)(8,47.21)(9,55.55)(10,59.72)};
       \legend{\textbf{\ours~(SDMQ)},\textbf{\wsup}}
       \end{axis}
   \end{tikzpicture}
}
\caption{
\small
\ours, in addition to being more effective than \wsup, also outperforms \wsup~in terms of training time because of a much smaller number of parameters (1.9M vs. 4.7M).}
\label{fig:epoch_vs_time}
\end{figure}


==> plotdefs/num_layer_accu.tex <==
\resizebox{1\columnwidth}{!}{
   \begin{tikzpicture}
       \begin{axis}[
           title={\textbf{(a) TREC-Robust}},
           xlabel={\textbf{Number of feed-forward layers}},
           ylabel={\textbf{Accuracy}},
           xmin=0.7, xmax=4.2,
           ymin=0.5, ymax=0.9,
           xtick={1,2,3,4},
           ytick={0.5,0.6,0.7,0.8,0.9,1},
           legend pos=north east,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=red,
           mark=square,
           ]
           coordinates {(1,0.8419)(2,0.7321)(3,0.7011)(4,0.6194)};
       %
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=x,
           ]
           coordinates {(1,0.8119)(2,0.6942)(3,0.6473)(4,0.5349)};
       \legend{\textbf{Depp-QPP(SD-MQ)},\textbf{WS-NeuralQPP}}
       \end{axis}
   \end{tikzpicture}
% 
\begin{tikzpicture}
       \begin{axis}[
           title={\textbf{(a) ClueWeb09}},
           xlabel={\textbf{Number of feed-forward layers}},
           ylabel={\textbf{Accuracy}},
           xmin=0.7, xmax=4.2,
           ymin=0.5, ymax=0.9,
           xtick={1,2,3,4},
           ytick={0.5,0.6,0.7,0.8,0.9,1},
           legend pos=north east,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=orange,
           mark=square,
           ]
           coordinates {(1,0.8042)(2,0.6918)(3,0.5836)(4,0.5764)};
       %
       \addplot[
           line width=0.5mm,
           color=blue,
           mark=x,
           ]
           coordinates {(1,0.7721)(2,0.6214)(3,0.5344)(4,0.5410)};
       \legend{\textbf{Depp-QPP(SD-MQ)},\textbf{WS-NeuralQPP}}
       \end{axis}
   \end{tikzpicture}
}
\begingroup
\captionof{figure}{Variation of model's performance with the change of number of layers in the fully connected network it is passed thorough as in the Figure \ref{fig:overview}. Comparison is shown between our proposed Deep-QPP(SD-MQ) approach and WS-NeuralQPP \cite{hamed_neuralqpp}.}\label{layer_vs_accu}
\endgroup


==> plotdefs/t-b-accuracy.tex <==
\begin{figure}[t]
\centering
\resizebox{1\columnwidth}{!}{
   \begin{tikzpicture}
       \begin{axis}[
           title={\textbf{(a) TREC-Robust}},
           xlabel={\textbf{$t$}},
           ylabel={\textbf{Accuracy}},
           xmin=0, xmax=20,
           ymin=0.2, ymax=1,
           xtick={0,5,10,15,20},
           ytick={0.2,0.4,0.6,0.8,1},
           legend pos=south east,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=black,
           mark=x,
           ]
           coordinates {(0,0.5873)(5,0.7341)(10,0.8037)(15,0.7529)(20,0.7082)};
       %
       \addplot[
           line width=0.5mm,
           color=blue,
           mark=square,
           ]
           coordinates {(0,0.4127)(5,0.8017)(10,0.7962)(15,0.7767)(20,0.7184)};
       %
       \addplot[
           line width=0.5mm,
           color=red,
           mark=o,
           ]
           coordinates {(0,0.4082)(5,0.7481)(10,0.8420)(15,0.7841)(20,0.6932)};
       %
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=x,
           ]
           coordinates {(0,0.4200)(5,0.7619)(10,0.7834)(15,0.7011)(20,0.6423)};
       %
       \addplot[
           line width=0.5mm,
           color=brown,
           mark=triangle,
           ]
           coordinates {(0,0.4276)(5,0.6731)(10,0.6279)(15,0.7214)(20,0.6149)};
       \legend{\textbf{$b$=0},\textbf{$b$=5},\textbf{$b$=10},\textbf{$b$=15},\textbf{$b$=20}}
       \end{axis}
   \end{tikzpicture}
% 
   \begin{tikzpicture}
       % \centering
       \begin{axis}[
           title={\textbf{(b) ClueWeb09}},
           xlabel={\textbf{$t$}},
           ylabel={\textbf{Accuracy}},
           xmin=0, xmax=20,
           ymin=0.2, ymax=1,
           xtick={0,5,10,15,20},
           ytick={0.2,0.4,0.6,0.8,1},
           legend pos=south east,
           xmajorgrids=true,
           ymajorgrids=true,
           grid style=dashed,
       ]
       
       \addplot[
           line width=0.5mm,
           color=black,
           mark=x,
           ]
           coordinates {(0,0.6015)(5,0.6734)(10,0.7659)(15,0.7077)(20,0.6840)};
       %   
       \addplot[
           line width=0.5mm,
           color=blue,
           mark=square,
           ]
           coordinates {(0,0.4003)(5,0.7415)(10,0.7698)(15,0.7532)(20,0.7128)};
       %
       \addplot[
           line width=0.5mm,
           color=red,
           mark=o,
           ]
           coordinates {(0,0.4330)(5,0.7627)(10,0.8045)(15,0.7019)(20,0.7191)};
       %
       \addplot[
           line width=0.5mm,
           color=cyan,
           mark=x,
           ]
           coordinates {(0,0.4211)(5,0.7018)(10,0.7932)(15,0.6734)(20,0.6032)};
       %
       \addplot[
           line width=0.5mm,
           color=brown,
           mark=triangle,
           ]
           coordinates {(0,0.4187)(5,0.6549)(10,0.7047)(15,0.6321)(20,0.6072)};
       \legend{\textbf{$b$=0},\textbf{$b$=5},\textbf{$b$=10},\textbf{$b$=15},\textbf{$b$=20}}
       \end{axis}
   \end{tikzpicture}
}
\caption{
\small
Sensitivity of \ours~on the number of top ($t$) and bottom ($b$) documents to include for interaction computation (see Section \ref{ss:qd-interaction}) on QPP effectiveness. The limiting case of $(t, b)=(0, 0)$ corresponds to the situation when we simply use the interaction between query terms themselves (i.e. the DRMM baseline).
\label{fig:t-b-accu}
}
\end{figure}


==> tabdefs/cw_res_summary.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{3pt}
%\resizebox{\columnwidth}{!}{

\begin{tabular}{lccccc}
\toprule
Method & \multicolumn{2}{c}{Parameters} & Pairwise & \multicolumn{2}{c}{Pointwise}
\\
\cmidrule{2-3}
\cmidrule{4-4}
\cmidrule{5-6}

 & $t$ & $b$ & Accuracy & P-$\mathscr{r}$ & K-$\tau$
\\

\midrule

AvgIDF & & & 0.7424 & 0.2440 & 0.1910
\\

MaxIDF & & & 0.6798 & 0.2013 & 0.1334
\\

Clarity & & & 0.6118 & 0.1906 & 0.0638
\\

NQC & & & 0.7032 & 0.2651 & 0.1503
\\

WIG & & & 0.6832 & 0.2492 & 0.1915
\\

UEF(NQC) & & & 0.7214 & 0.3159	& 0.1962
\\

\midrule

BERT &  &  & 0.6892 & 0.2312 & 0.1439
\\

Vec-sum &  &  & 0.6271 & 0.2104 & 0.1156
\\

LSTM-vec &  &  & 
\\

Query-query &  &  & 0.6015 & 0.2011 & 0.1137
\\

NeuralQPP \cite{hamed_neuralqpp} & 10 & 0 & 0.7721 & 0.5189 & 0.2823
\\

\midrule

MD-MQ & 10 & 0 & 0.7269 & 0.4258 & 0.2374
\\

MD-MQ & 10 & 10 & 0.7410 & 0.4632 & 0.2490
\\

SD-MQ & 10 & 0 & 0.7659 & 0.4962 & 0.2730
\\

SD-SQ & 10 & 10 & 0.6849 & 0.4211 & 0.2400
\\

MD-SQ & 10 & 0 & 0.7400 & 0.4691 & 0.2550
\\

MD-SQ & 10 & 10 & 0.7429 & 0.4846 & 0.2578
\\

% \midrule

SD-MQ & 10 & 10 & \textbf{0.8042} & \textbf{0.5529} & \textbf{0.3124}
\\

\bottomrule
                       
\end{tabular}
%}
\caption{
%\small
Results obtained through $5$-fold cross-validation for all the supervised and unsupervised methods as in Table \ref{tab:results_summary_trec} on ClueWeb09 dataset. Parameters $t$ and $b$ have the same meaning as mentioned in Table \ref{tab:results_summary_trec}. Our proposed SD-MQ performs the best over all other methods significantly (t-test with 95\% confidence) obtaining 80\% accuracy and Pearson's rank correlation value of 0.5529.
}
\label{tab:results_summary_cw}
\end{table}

==> tabdefs/idf_ablation.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{

\begin{tabular}{l ccc|ccc}
\toprule
& \multicolumn{3}{c}{TREC-Robust} & \multicolumn{3}{c}{ClueWeb09}
\\
\cmidrule{2-4}
\cmidrule{5-7}

Methods & Pairwise & \multicolumn{2}{c}{Pointwise} & Pairwise & \multicolumn{2}{c}{Pointwise}
\\

\cmidrule{2-2}
\cmidrule{3-4}
\cmidrule{5-5}
\cmidrule{6-7}

& Accuracy & P-$\mathscr{r}$ & K-$\tau$ & Accuracy & P-$\mathscr{r}$ & K-$\tau$
\\
\midrule

% MD-MQ & 10 & 0 & 0.7016 & 0.6249 & 0.3951 & 0.6451 & 0.3619 & 0.2011
% \\

MD-MQ & 0.7096 & 0.6344 & 0.4272 & 0.7003 & 0.4062 & 0.1996
\\

% SD-MQ & 10 & 0 & 0.7611 & 0.6702 & 0.4328 & 0.6862 & 0.4538 & 0.2513
% \\

SD-SQ & 0.6500 & 0.5762 & 0.3701 & 0.6133 & 0.3817 & 0.1794
\\

% MD-SQ & 10 & 0 & 0.7152 & 0.6390 & 0.4219 & 0.6827 & 0.3912 & 0.2102
% \\

MD-SQ & 0.7309 & 0.6721 & 0.4361 & 0.6683 & 0.4221 & 0.2018
\\

SD-MQ & 0.7472 & 0.6744 & 0.4621 & 0.7519 & 0.4839 & 0.2780
\\

\bottomrule
                       
\end{tabular}
}

\caption{
%\small
Without idf
}
\label{tab:res_table_merge}
\end{table}

==> tabdefs/merged_table_res.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{3pt}
%\resizebox{\columnwidth}{!}{

\begin{tabular}{l ccc ccc|ccc}
\toprule
& \multicolumn{3}{c}{Deep-QPP} & \multicolumn{3}{c}{TREC-Robust} & \multicolumn{3}{c}{ClueWeb09}
\\
\cmidrule{5-7}
\cmidrule{8-10}

Methods & \multicolumn{3}{c}{Parameters} & Pairwise & \multicolumn{2}{c}{Pointwise} & Pairwise & \multicolumn{2}{c}{Pointwise}
\\

\cmidrule{2-4}
\cmidrule{5-5}
\cmidrule{6-7}
\cmidrule{8-8}
\cmidrule{9-10}

& $\pi$ & $t$ & $b$ & Accuracy & P-$\mathscr{r}$ & K-$\tau$ & Accuracy & P-$\mathscr{r}$ & K-$\tau$
\\
\midrule

% AvgIDF & & & 0.7811 & 0.6984 & 0.4873 & 0.7424 & 0.2440 & 0.1910
% \\

% MaxIDF & & & 0.7078 & 0.6329 & 0.4759 & 0.6798 & 0.2013 & 0.1334
% \\

Clarity & - & - & - & 0.6242 & 0.4881 & 0.3140 & 0.6118 & 0.1906 & 0.0638
\\

NQC & - & - & - & 0.6718 & 0.5272 & 0.4038 & 0.7032 & 0.2651 & 0.1503
\\

WIG & - & - & - & 0.6600 & 0.5437 & 0.4286 & 0.6832 & 0.2492 & 0.1915
\\

UEF(WIG) & - & - & - & 0.6943 & 0.5519 & 0.4152 & 0.7214 & 0.3159	& 0.1962
\\

\midrule

SN-BERT & - & - & - & 0.6619 & 0.5211 & 0.4172 & 0.6892 & 0.2312 & 0.1439
\\

SN-Skipgram & - & - & - & 0.6349 & 0.5112 & 0.3987 & 0.6271 & 0.2104 & 0.1156
\\

% LSTM-vec &  &  & 
% \\

Query-Query Interaction & - & - & - & 0.5873 & 0.4728 & 0.3712 & 0.6015 & 0.2011 & 0.1137
\\

WS-NeurQPP \cite{hamed_neuralqpp} & - & 10 & 0 & 0.8119 & 0.7218 & 0.5089 & 0.7721 & 0.5189 & 0.2823
\\

\midrule
\midrule

% MD-MQ & 10 & 0 & no & 
% \\

% MD-MQ & 10 & 10 & no &
% \\

% SD-MQ & 10 & 0 & no &
% \\

% SD-SQ & 10 & 10 & no &
% \\

% MD-SQ & 10 & 0 & no &
% \\

% MD-SQ & 10 & 10 & no &
% \\

% SD-MQ & 10 & 10 & no &
% \\

% \midrule

% Deep-QPP & MD-MQ & 10 & 0 & 0.7531 & 0.6612 & 0.4257 & 0.7269 & 0.4258 & 0.2374
% \\

Deep-QPP & MD-MQ & 10 & 10 & 0.7857 & 0.6987 & 0.4983 & 0.7410 & 0.4632 & 0.2490
\\

% Deep-QPP & SD-MQ & 10 & 0 & 0.8037 & 0.7204 & 0.5097 & 0.7659 & 0.4962 & 0.2730
% \\

Deep-QPP & SD-SQ & 10 & 10 & 0.7212 & 0.6300 & 0.4020 & 0.6849 & 0.4211 & 0.2400
\\

% Deep-QPP & MD-SQ & 10 & 0 & 0.7893 & 0.7002 & 0.4900 & 0.7400 & 0.4691 & 0.2550
% \\

Deep-QPP & MD-SQ & 10 & 10 & 0.8004 & 0.7200 & 0.4992 & 0.7429 & 0.4846 & 0.2578
\\

Deep-QPP & SD-MQ & 10 & 10 & \textbf{0.8419} & \textbf{0.7402} & \textbf{0.5432} & \textbf{0.8042} & \textbf{0.5529} & \textbf{0.3124}
\\

\bottomrule
                       
\end{tabular}
%}
\caption{
%\small
\input{tabdefs/results_caption}
}
\label{tab:res_table_merge}
\end{table*}

==> tabdefs/results.tex <==
\begin{table}[t]
\centering
\small

\begin{tabular}{@{}l@{~}r@{~~}r@{~~}r|r@{~~}r@{~~}r@{}}

%\begin{tabular}{l ccccc|ccccc}
\toprule
& \multicolumn{3}{c}{TREC-Robust} & \multicolumn{3}{c}{ClueWeb09}\\

\cmidrule(r){2-4}
\cmidrule(l){5-7}


Methods  & \multicolumn{1}{c}{Pairwise} & \multicolumn{2}{c}{Pointwise} & \multicolumn{1}{c}{Pairwise} & \multicolumn{2}{c}{Pointwise}\\

\cmidrule(r){2-4}
\cmidrule(l){5-7}

& Accuracy & P-$\rho$ & K-$\tau$ 
& Accuracy & P-$\rho$ & K-$\tau$
\\

\midrule

% AvgIDF & & & 0.7811 & 0.6984 & 0.4873 & 0.7424 & 0.2440 & 0.1910
% \\

% MaxIDF & & & 0.7078 & 0.6329 & 0.4759 & 0.6798 & 0.2013 & 0.1334
% \\

Clarity & 0.6242 & 0.4881 & 0.3140 
& 0.6118 & 0.1906 & 0.0638
\\

NQC & 0.6718 & 0.5272 & 0.4038 
& 0.7032 & 0.2651 & 0.1503
\\

WIG & 0.6600 & 0.5437 & 0.4286 
& 0.6832 & 0.2492 & 0.1915
\\

UEF & 0.6943 & 0.5519 & 0.4152 
& 0.7214 & 0.3159	& 0.1962
\\

\midrule

SN-BERT & 0.6619 & 0.5211 & 0.4172 
& 0.6892 & 0.2312 & 0.1439
\\

SN-SG & 0.6349 & 0.5112 & 0.3987 
& 0.6271 & 0.2104 & 0.1156
\\

% LSTM-vec &  &  & 
% \\

DRMM & 0.5873 & 0.4728 & 0.3712 
& 0.6015 & 0.2011 & 0.1137\\

\wsup & 0.8119 & 0.7218 & 0.5089 
& 0.7721 & 0.5189 & 0.2823\\

\midrule

Deep-QPP (MDMQ) & 0.7857 & 0.6987 & 0.4983 
& 0.7410 & 0.4632 & 0.2490\\

Deep-QPP (SDSQ) & 0.7212 & 0.6300 & 0.4020 
& 0.6849 & 0.4211 & 0.2400\\

Deep-QPP (MDSQ) & 0.8004 & 0.7200 & 0.4992 
& 0.7429 & 0.4846 & 0.2578
\\

Deep-QPP (SDMQ) & \textbf{0.8419} & \textbf{0.7402} & \textbf{0.5432}  & \textbf{0.8042}  & \textbf{0.5529} & \textbf{0.3124} \\

\bottomrule
                       
\end{tabular}
%}
\caption{
%\small
A comparison of the QPP effectiveness between \ours, and a set of unsupervised and supervised baselines - the 1$^{st}$ and 2$^{nd}$ groups, respectively.
The \hlt{average} accuracy \hlt{(see `Metrics' in Section \ref{ss:evalmetrics})} and the correlation values of \ours~over the best performing baseline - \wsup, is statistically significant (t-test with over 97\% confidence). The percentage improvements of \ours~(SDMQ) relative to \wsup~are \emph{higher for the web queries} (e.g., 6.55\% vs. 2.55\% improvement in $\rho$ for ClueWeb and TREC-Rb, respectively).
}
\label{tab:res_table_merge}
\end{table}

==> tabdefs/trec_res_summary.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{3pt}
%\resizebox{\columnwidth}{!}{

\begin{tabular}{lccccc}
\toprule
Method & \multicolumn{2}{c}{Parameters} & Pairwise & \multicolumn{2}{c}{Pointwise}
\\
\cmidrule{2-3}
\cmidrule{4-4}
\cmidrule{5-6}

 & $t$ & $b$ & Accuracy & P-$\mathscr{r}$ & K-$\tau$
\\

\midrule

AvgIDF & & & 0.7811 & 0.6984 & 0.4873
\\

MaxIDF & & & 0.7078 & 0.6329 & 0.4759
\\

Clarity & & & 0.6242 & 0.4881	& 0.3140
\\

NQC & & & 0.6718 & 0.5272	& 0.4038
\\

WIG & & & 0.6600 & 0.5437 & 0.4286
\\

UEF(WIG) & & & 0.6943 & 0.5519 & 0.4152
\\

\midrule

BERT &  &  & 0.6619 & 0.5211 & 0.4172
\\

Vec-sum &  &  & 0.6349 & 0.5112 & 0.3987 
\\

LSTM-vec &  &  & 
\\

Query-query &  &  & 0.5873 & 0.4728 & 0.3712
\\

NeuralQPP \cite{hamed_neuralqpp} & 10 & 0 & 0.8119 & 0.7218 & 0.5089
\\

\midrule

MD-MQ & 10 & 0 & 0.7531 & 0.6612 & 0.4257
\\

MD-MQ & 10 & 10 & 0.7857 & 0.6987 & 0.4983
\\

SD-MQ & 10 & 0 & 0.8037 & 0.7204 & 0.5097
\\

SD-SQ & 10 & 10 & 0.7212 & 0.6300 & 0.4020
\\

MD-SQ & 10 & 0 & 0.7893 & 0.7002 & 0.4900
\\

MD-SQ & 10 & 10 & 0.8004 & 0.7200 & 0.4992
\\

% \midrule

SD-MQ & 10 & 10 & \textbf{0.8419} & \textbf{0.7402} & \textbf{0.5432}
\\

\bottomrule
                       
\end{tabular}
%}
\caption{
%\small
Both pairwise (with accuracy) and pointwise (with rank correlation values measured by Pearson's-$\mathscr{r}$ and Kendall's-$\tau$) estimations on TREC-Robust dataset. We report $5$-fold cross-validated results for each of the techniques. 
Parameters $t$ and $b$ are only applicable for \emph{interaction}-based supervised models denoting the number of top set and the bottom set of documents respectively taken from a larger set of documents $\{D\}$, where $|D|$ > $|t|+|b|$, used for interaction generation. Bold-faced numbers indicate that our proposed SD-MQ ($t=10,b=10$) outperforms all other methods with 84\% accuracy and also the rank correlation value improves significantly over other QPP approaches (t-test with 98\% confidence).
}
\label{tab:results_summary_trec}
\end{table}
